Effects of Cosine Tapering Window on Quantum Phase Estimation

We provide a modification to the quantum phase estimation algorithm (QPEA) inspired on classical windowing methods for spectral density estimation. From this modification we obtain an upper bound in the cost that implies a cubic improvement with respect to the algorithm's error rate. Numerical evaluation of the costs also demonstrates an improvement. Moreover, with similar techniques, we detail an iterative projective measurement method for ground state preparation that gives an exponential improvement over previous bounds using QPEA. Numerical tests that confirm the expected scaling behavior are also obtained. For these numerical tests we have used a Lattice Thirring model as testing ground. Using well-known perturbation theory results, we also show how to more appropriately estimate the cost scaling with respect to state error instead of evolution operator error.

==> tikzlibraryquantikz.code.tex <==
%auto-ignore
%This is the quantikz library for typesetting quantum circuits using LaTeX/Tikz. version 0.9.4
% Written by Alastair Kay, 2018. Published under a CC-BY-4.0 licence
% Please email me (alastair.kay@rhul.ac.uk) with any bug reports or feature requests.
% If you find this library useful, please cite its usage in your work, using arXiv:1809.03842, and possibly the DOI: 10.17637/rh.7000520.
% Usage is at your own risk.

%version 0.9.5:
%	fixed bug which meant multi-wire gates didn't work outside of an environment such as center.
%version 0.9.4:
%	added nwires and cwires options to gate command to simulate qcircuit's nphantom and cphantom
%	vertical text options for slice labels.
%	replaced macro for measuring width and height for greater reliability. disable auto spacing now unnecessary as things like \sqrt{} work in the gate label.
%	investigated possibility of high labels (multi-line labels, particularly for a multi-qubit gate). key disable auto height introduced.
%	now provides a quantikz environment, which is theoretically compatible with tikz' external library (entirely untested). Can still use tikzcd environment otherwise.
%	removed a tikzcd customisation fixing the baseline for one row circuits as this was messing with any manual attempts to adjust the baseline.
%version 0.9.3:
%	adjusted spacing of gate operation between in-circuit and overlay so that transparency looks better
%	Other gate spacing adjustments. multi-qubit gates in particular should look better. 'disable auto spacing' can switch this off, particularly for use with things like \sqrt{} in the multi-qubit gate label, which will throw a weird error.
%	gate command now takes two further optional parameters: minimum width and minimum height for each cell.
%	some consolidation of styling commands
%	global keys 'transparent' and 'thin lines' added. 'thin lines' gives a look more similar to the original QCircuit.
%version 0.9.2:
%	made 'wires' the default key, so [wires=2] now becomes [2]
%	added 'slice title', 'slices style', 'slices label style' key to control titles of slices under 'slice all'
%	better access to positioning of gategroup label.
%	now arXiv compatible (that was a challenge! they use old versions of packages)
%Previous versions:
%version 0.9.1:
%	added \cwbend gate for cornering classical wires.
%	made size of strike through for multiqubit gates stylable via the keys /quantikz/Strike Height/ and /quantikz/Strike Width/
%	added new \gate[swap] variant of swap (nearest-neighbour only).
%version 0.9.0:
%original release.

\ProvidesPackage{quantikz}[2019/04/24 typeset quantum circuit diagrams]

% Package(s) to include
\RequirePackage{xargs,ifthen,xstring,xparse,etoolbox,mathtools}
\RequirePackage{environ} %in an attempt to help with compatibility with the external library of tikz.
\RequirePackage{tikz}
\usetikzlibrary{cd,decorations.pathreplacing,calc,positioning,fit,shapes.symbols,decorations.pathmorphing,shapes.misc,backgrounds,decorations.markings}

\newlength{\myl}
\newlength{\myh}
\newlength{\myd}

%\makeatletter
\newcounter{aaa}
\tikzset{
  apply/.style args={#1 except on segments #2}{postaction={
      /utils/exec={
        \@for\mattempa:=#2\do{\csdef{aaa@\mattempa}{}}
        \setcounter{aaa}{0}
      },
      decorate,decoration={show path construction,
        moveto code={},
        lineto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path[#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
        curveto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) .. controls
            (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
            ..(\tikzinputsegmentlast);
          }
        },
        closepath code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
      },
    },
  },
}
%test if item is in list of item. Probably better ways to do this, but I could get this version to work.
\newcommand*{\IfInList}[2]{%
	\gdef\memory{0}
	\edef\arg{#1}
	 \foreach \q in #2 {%
	 	\ifthenelse{\q=\arg}{%
	 		\gdef\memory{1}
	 	}{}
	 }
	\ifthenelse{\memory=1} {%
		\expandafter\@firstoftwo
	}{%
		\expandafter\@secondoftwo
	}
}
%define the quantikz environment. I need this to facilitate the external library
\NewEnviron{quantikz}[1][]{%
  \def\@temp{\tikzcd@[#1]\BODY}%
  \expandafter\@temp\endtikzcd
}
\def\temp{&} \catcode`&=\active \let&=\temp
%
%commands for putting in text vertically
\protected\def\vvv#1{\leavevmode\bgroup\vbox\bgroup\xvvv#1\relax}
%
\def\xvvv{\afterassignment\xxvvv\let\tmp= }
%
\def\xxvvv{%
% \ifx\tmp\@sptoken\egroup\ \vbox\bgroup\let\next\xvvv
% \else
\ifx\tmp\relax\egroup\egroup\let\next\relax
 \else
\hbox to 1.1em{\hfill\tmp\hfill}% centred
\let\next\xvvv\fi%\fi
\next}
%end of commands for putting text vertically
%
\long\def\ifnodedefined#1#2#3{%
    \@ifundefined{pgf@sh@ns@#1}{#3}{#2}%
}
%I don't think this is used any more
% \newcommand\getwidth[1]{
% 	\pgfkeys{minimum width=0pt}%
% 	\pgfkeys{/quantikz,#1}
% 	\pgfkeysgetvalue{/quantikz/minimum width}{\minwidth}
% 	\minwidth
% }

%the main gate command
\DeclareExpandableDocumentCommand{\gate}{O{}O{1.5pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner sep=4pt,minimum width=#2,minimum height=#3]|%
 	\edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
 	%reset macros that are going to be set by the options
 	\edef\options{row=\n,col=\m,#1}
 	\def\toswap{0}%
 	\def\DisableMinSize{0}%
 	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
 	%import options passed as parameters
  	\pgfkeys{/quantikz,#1}%
 	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
 	\pgfkeysgetvalue{/quantikz/style}{\a}
 	\pgfkeysgetvalue{/quantikz/label style}{\b}
 	\pgfkeysgetvalue{/quantikz/cwires}{\mylist}
 	\pgfkeysgetvalue{/quantikz/nwires}{\nowires}
 	\ifthenelse{\toswap=1}{%if it's a swap gate...
 		\def\quantwires{2}
 		\phantom{wide}
 		\settowidth{\myl}{$wide$}
 		\settoheight{\myh}{$wide$}
 		\settodepth{\myd}{$wide$}
 	}{%not a swap gate
 		\settowidth{\myl}{$#4$}
 		\ifthenelse{\DisableMinSize=1}{%disable automatic size detection. Use $U$ instead.
 			\phantom{U}
 			\settoheight{\myh}{$U$}
 			\settodepth{\myd}{$U$}
 		}{%automatically get width and height of label
 			\phantom{#4}
 			\settoheight{\myh}{$#4$}
 			\settodepth{\myd}{$#4$}
 		}
 	}
%	
 	\IfInList{1}{\mylist}{\cw}{\IfInList{1}{\nowires}{}{\qw}}%do we need classical, no wire, or quantum wire?
 	\edef\k{\the\numexpr\n+\quantwires-1\relax}
 	\edef\mn{\the\numexpr\m-1\relax}
 	\ifthenelse{\quantwires=1}{}{%more than 1 wire on gate. iterate through each wire
 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
 	    \edef\newcom{\noexpand\vcwhexplicit{\i-\m}{\i-\mn}}
       	\edef\newcomb{\noexpand\vqwexplicit{\i-\m}{\i-\mn}}
 	 	\edef\val{\the\numexpr\i+1-\n\relax}
 		\IfInList{\val}{\mylist}{\newcom}{\IfInList{\val}{\nowires}{}{\newcomb}}%do we need classical, no wire, or quantum wire?
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
 		\globaldefs=1
 		\edef\dotikzset{\noexpand\tikzset{row \i\space column \m/.append style={minimum width={max(\the\myl+8pt,#2)}}}}
 		\dotikzset
 		\edef\undotikzset{\noexpand\tikzset{row \i\space column \m/.style={}}}
      	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendglobals\expandafter{\undotikzset}
 	}
 			%apply auto height to last row only. unsetting already handled above.
 		   \globaldefs=1
 		   \edef\dotikzset{\noexpand\tikzset{row \k\space column \m/.append style={minimum height={max(\the\myh+\the\myd+8pt,#3)}}}}
 		   \dotikzset
%		
 	}
 	%call deferred gate command.
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gate@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\a\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\b\expandafter}\expandafter{\options}{#4}
	}
}

%deferred gate command. draws a box around all included cells. this is not part of the matrix, but comes afterwards.
\newcommand{\gate@end}[4]{
	\pgfkeys{/quantikz,wires=1}
	\def\toswap{0}
	\def\DisableMinSize{0}
 	\pgfkeys{/quantikz,#3}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\ifthenelse{\toswap=1}{\def\quantwires{2}}{}
	\xdef\LoopGG{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGG{\LoopGG(\tikzcdmatrixname-\n-\col)}
		}{}
	}
	\ifthenelse{\toswap=1}{
		\node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,#1] {\hphantom{Wide}};
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\row-\col.center) to[out=0,in=180] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [line width=3pt,white,shorten >=0.9pt,shorten <=0.9pt] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
	}{
	  \node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,label={[gg label,#2]$#4$},#1] {\hphantom{$#4$}};
	}
}

%ghost will get height correct if can't be automatically assigned.
\DeclareExpandableDocumentCommand{\ghost}{O{}O{0pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner ysep=4pt,minimum width=#2,minimum height=#3]| \vphantom{#4}
}


%single slice
\newcommand\slice[2][]{%
	%\edef\currcol{\the\pgfmatrixcurrentcolumn}
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
 	\edef\options{\pgfkeysvalueof{/quantikz/style}}
 	\edef\opts{\pgfkeysvalueof{/quantikz/label style}}
	\edef\n{\the\pgfmatrixcurrentcolumn}
	%\expandafter\show\n
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendslices\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}}
%deferred slice command
\newcommand{\slice@end}[4]{
	\edef\top{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row1.north)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row1.north)$)}
	\edef\bottom{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+(0,-3pt)$)}
	\expandafter\expandafter\expandafter\make@slice\expandafter\expandafter\expandafter{\expandafter\top\expandafter}\expandafter{\bottom}{#4}{#2}{#3}
}
\newcommand{\make@slice}[5]{
	\draw[slice,#4] #1 to node[pos=0,inner sep=4pt,anchor=south,color=black,#5] {#3} #2;
}
%deferred command which will slice everything
\newcommand{\sliceallr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\pgfkeysvalueof{/tikz/slice titles}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}
%deferred slice command with vertical text
\newcommand{\sliceallvr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\vvv{\pgfkeysvalueof{/tikz/slice titles}}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}

%labelling of inputs
\newcommand\lstick[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupinput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%labelling of outputs
\newcommand\rstick[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred labelling of inputs
\newcommand{\groupinput@end}[4]{%basic data as keys, lable options, brace options, text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGI{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGI{\LoopGI(\tikzcdmatrixname-\n-\col)} 
		}{}
		}
	\ifthenelse{\quantwires=1} {
		\node (ingr-\row) [fit=\LoopGI, inner sep=0pt,label={[align=center,#2]left:#4}] {};
	}{
	\node (ingr-\row) [fit=\LoopGI, inner sep=0pt] {};
	\draw[dm,#3] ($(ingr-\row.north west)+(-0.1cm,0.1cm)$) to node[midway,align=center,anchor=east,xshift=-0.1cm,#2] {#4} ($(ingr-\row.south west)+(-0.1cm,-0.1cm)$);
	}
} %
%deferred labelling of outputs
\newcommand{\groupoutput@end}[4]{%basic data as keys, lable options, brace options, text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGO{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
		\ifnodedefined{\tikzcdmatrixname-\n-\col}{
			\xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\col)} 
		}}
		\ifthenelse{\quantwires=1} {
		\node (outgr-\row) [fit=\LoopGO, inner sep=0pt,label={[align=center,#2]right:#4}] {};
	}{
	\node (outgr-\row) [fit=\LoopGO, inner sep=0pt] {};
	\draw[dd,#3] ($(outgr-\row.north east)+(0.1cm,0.1cm)$) to node[midway,align=center,anchor=west,xshift=0.1cm,#2] {#4} ($(outgr-\row.south east)+(0.1cm,-0.1cm)$);
	}
} %
%inputs and outputs within a multi-wire gate
\newcommand\gateinput[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/braces}{\opts}%
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mginput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
\newcommand\gateoutput[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mgoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred functions for the above
\newcommand{\mginput@end}[4]{%collected options,label style, brace style,text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0,0cm)$)[leftinternal,#2]{#4};
}{%
%\show\quantwires
\draw[dd,#3] ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0.1cm,0.1cm)$) to node[leftinternal,midway,#2] {#4} ($(\cell.west |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.west)+(0.1cm,-0.1cm)$);
}
} %
\newcommand{\mgoutput@end}[4]{%
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(0,0cm)$)[rightinternal,#2]{#4};
}{%
\draw[dm,#3] ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(-0.1cm,0.1cm)$) to node[rightinternal,midway,#2] {#4} ($(\cell.east |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.east)+(-0.1cm,-0.1cm)$);
}
} %

%wave command
\newcommand\wave[1][]{%
	\edef\n{\the\pgfmatrixcurrentrow}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendslices\expandafter{%
		\expandafter\wave@end\expandafter{\n}{#1}%
	}
}
%deferred wave
\newcommand{\wave@end}[2]{
	\node (wave-#1) [fit=(\tikzcdmatrixname-row#1),wave,#2] {};
}

%put a border around a group of gates
\newcommand\gategroup[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/style}{\options}
 	\pgfkeysgetvalue{/quantikz/label style}{\opts}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gategroup@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred gate group command
\newcommand{\gategroup@end}[4]{%options, gate style, text style, text
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=,steps=1}%
	\edef\background{0}%
	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}%
	\pgfkeysgetvalue{/quantikz/row}{\row}%
	\pgfkeysgetvalue{/quantikz/col}{\col}%
	\pgfkeysgetvalue{/quantikz/steps}{\steps}%
	\edef\fit{(\tikzcdmatrixname-col\col.west |- \tikzcdmatrixname-row\row.north)(\tikzcdmatrixname-col\the\numexpr\col+\steps-1\relax.east |- \tikzcdmatrixname-row\the\numexpr\row+\quantwires-1\relax.south)}%
	\ifthenelse{\background=1}{%
		\begin{scope}[on background layer]\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};\end{scope}
	}{%
		\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};
	}
}

%use for fudging classical wires that have horizontal and vertical sections
\newcommand{\cwbend}[1]{
	\vcw{#1}\cw
	\edef\cell{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendlabels\expandafter{%
		\expandafter\latephase@end\expandafter{\cell}
	}
}

\newcommand{\latephase@end}[1]{
	\node [phase,inner sep=2pt] at (\tikzcdmatrixname-#1) {};
}

%patch tikzcd to allow for multiple layers of commands
\patchcmd\tikzcd@{\tikzpicture}{\def\toslice{0}\def\vert{0}
 \begin{tikzpicture}}{}{}
\patchcmd\tikzcd@
    {\global\let\tikzcd@savedpaths\pgfutil@empty}
    {\global\let\tikzcd@savedpaths\pgfutil@empty
    \global\let\tikzcd@atendsavedpaths\pgfutil@empty
    \global\let\tikzcd@atendlabels\pgfutil@empty
    \global\let\tikzcd@atendslices\pgfutil@empty
    \global\let\tikzcd@atendglobals\pgfutil@empty
    \pgfutil@g@addto@macro\tikzcd@savedpaths\DivideRowsCols
    %\pgfmathsetmacro{\mname}{random(100000)}
    \ifthenelse{\toslice=1}{\ifthenelse{\vert=0}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallr}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallvr}}{}
    }{}{}

%this patching works on modern systems, but I believe is incompatible with the old version that arXiv is running
%\patchcmd\endtikzcd{\tikzcd@savedpaths}{\tikzcd@savedpaths\tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices{\globaldefs=1\tikzcd@atendglobals}}{}{}

%instead, completely redefine the function
\def\endtikzcd{%
  \pgfmatrixendrow\egroup%
  \pgfextra{\global\let\tikzcdmatrixname\tikzlastnode};%
  \tikzcdset{\the\pgfmatrixcurrentrow-row diagram/.try}%
  \begingroup%
    \pgfkeys{% `quotes' library support
      /handlers/first char syntax/the character "/.initial=\tikzcd@forward@quotes,%
      /tikz/edge quotes mean={%
        edge node={node [execute at begin node=\iftikzcd@mathmode$\fi,%$
                         execute at end node=\iftikzcd@mathmode$\fi,%$
                         /tikz/commutative diagrams/.cd,every label,##2]{##1}}}}%
    \let\tikzcd@errmessage\errmessage% improve error messages
    \def\errmessage##1{\tikzcd@errmessage{##1^^J...^^Jl.\tikzcd@lineno\space%
        I think the culprit is a tikzcd arrow in cell \tikzcd@currentrow-\tikzcd@currentcolumn}}%
    \tikzcd@before@paths@hook%
    \tikzcd@savedpaths\tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices{\globaldefs=1\tikzcd@atendglobals}%I just added stuff here instead
  \endgroup%
  \end{tikzpicture}%
  \ifnum0=`{}\fi}


%end patching
%\makeatother

%this command runs after we've finished the matrix, and makes unified cells for each row and each column. This allows much nicer alignment of large boxes.
\newcommand{\DivideRowsCols}{
	\foreach \n in {1,...,\the\pgfmatrixcurrentrow} {%for each row, construct a master cell that contains all entries
	\xdef\LoopRow{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentcolumn}{
			\ifnodedefined{\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(\tikzcdmatrixname-\n-\m)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(group\tikzcdmatrixname-\n-\m)}
			}{}
	}
	\node (\tikzcdmatrixname-row\n) [fit=\LoopRow] {};
	}
	\foreach \n in {1,...,\the\pgfmatrixcurrentcolumn} {%for each column, construct a master cell that contains all entries
	\xdef\LoopCol{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentrow}{
			\ifnodedefined{\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(\tikzcdmatrixname-\m-\n)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(group\tikzcdmatrixname-\m-\n)}
			}{}
	}
	\node (\tikzcdmatrixname-col\n) [fit=\LoopCol] {};
	}
}

%initialise all the pgfkeys for key=value parametre passing in macro options

\pgfkeys{/tikz/slice all/.code={\def\toslice{1}},/tikz/remove end slices/.initial=0,/tikz/slice titles/.initial={\col},/tikz/slice style/.initial={},/tikz/slice label style/.initial={},/tikz/thin lines/.code={\resetstyles},/tikz/transparent/.code={\maketransparent},/tikz/vertical slice labels/.code={\def\vert{1}}}
\pgfkeys{/quantikz/.is family,/quantikz,%
.unknown/.style={%
	/quantikz/wires=\pgfkeyscurrentname
},%
wires/.initial=1,%
style/.initial={},label style/.initial={},braces/.initial={},background/.code={\def\background{1}},alternate/.code={\def\helper{1}},row/.initial=1,col/.initial=1,steps/.initial=1,Strike Width/.initial=0.08cm,Strike Height/.initial=0.12cm,swap/.code={\def\toswap{1}},disable auto height/.code={\def\DisableMinSize{1}},cwires/.initial={-1},nwires/.initial={-1}}

%my standard Dirac notation commands. can be overridden by user.
\providecommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}
\providecommand{\bra}[1]{\ensuremath{\left\langle#1\right |}}
\providecommand{\proj}[1]{\ensuremath{\ket{#1}\!\bra{#1}}}
\providecommand{\braket}[2]{\ensuremath{\left\langle#1\middle|#2\right\rangle}}

%single qubit operations
\newcommand{\phantomgate}[1]{|[linecont,thickness, inner ysep=3pt]| \phantom{#1} \qw}
\newcommand{\hphantomgate}[1]{|[linecont,minimum size=1.5em,thickness]| \hphantom{#1} \qw}
\newcommand{\push}[1]{#1 \qw}
\newcommand{\alias}[1]{|[alias=#1]|}
\DeclareExpandableDocumentCommand{\phase}{O{}m}{|[phase,#1,label={[phase label,#1]#2}]| {} \qw}
\DeclareExpandableDocumentCommand{\control}{O{}m}{|[phase,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\ocontrol}{O{}m}{|[ophase,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\targ}{O{}m}{|[circlewc,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\targX}{O{}m}{|[crossx2,#1]| {} \qw}
\newcommand{\linethrough}{|[linecont, inner ysep=3pt]| }

%measuring
\DeclareExpandableDocumentCommand{\meter}{O{}{m}}{|[meter,label={[my label]#2},#1]| {} \qw}
\DeclareExpandableDocumentCommand{\measuretab}{O{}{m}}{|[measuretab,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\meterD}{O{}{m}}{|[meterD,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\measure}{O{}{m}}{|[measure,#1]| {#2} \qw}

%controlled gates
\def\ctrl#1{\control{}	\vqw{#1}}
\def\octrl#1{\ocontrol{}\vqw{#1}}
\def\swap#1{%
	\targX{}
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vqwexplicitcenter\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}

%vertical wires
%classical vertical wire, relative positioning
\newcommand{\vcw}[1]{
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vcwexplicit\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}
%vertical quantum wire, relative positioning
\newcommand{\vqw}[1]{
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vqwexplicit\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}
%quantum wire, absolute positioning
\newcommand{\vqwexplicit}[2]{
	\arrow[from=#1,to=#2,arrows] {}
}
%classical vertical wire, absolute positioning
\newcommand{\vcwexplicit}[2]{
	\arrow[from=#1,to=#2,arrows,xshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,xshift=-0.05cm] {}
}
%classical horizontal wire, absolute positioning
\newcommand{\vcwhexplicit}[2]{
	\arrow[from=#1,to=#2,arrows,yshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.05cm] {}
}
%quantum wire, absolute positioning, going to centres of cell, not edge.
\newcommand{\vqwexplicitcenter}[2]{
	\arrow[from=#1,to=#2,arrows,start anchor=center,end anchor=center] {}
}

%horizontal wires
\newcommand{\qw}{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{\arrow[arrows]{l}}{}}
\newcommand{\cw}{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{\arrow[arrows,yshift=0.05cm]{l}\arrow[arrows,yshift=-0.05cm]{l}}{}}
%define the strike distance for strike-through on qwbundle.
%\newcommand*{\StrikeDistance}{0.1cm}%
%a bundle of horizontal quantum wires
\newcommand{\qwbundle}[2][]{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{
	\def\helper{0}
	\pgfset{/quantikz,#1}
	\ifthenelse{\helper=1}{
		\arrow[arrows,yshift=0.1cm]{l}\arrow[arrows]{l}\arrow[arrows,yshift=-0.1cm]{l}
	}{
	\arrow[phantom,strike arrow]{l}[xshift=\pgfkeysvalueof{/quantikz/Strike Width}, yshift=\pgfkeysvalueof{/quantikz/Strike Height},anchor=south west,inner sep=0pt]{\scriptstyle #2}
	}}{}}




%configure some of the style properties.
\tikzcdset{row sep/normal=0.5cm,column sep/normal=0.5cm,thick,nodes in empty cells,
	every cell/.style={
        anchor=center,minimum size=0pt,inner sep=0pt,outer sep=0pt,thick
    },
    arrows/.style={dash,thick},
    1-row diagram/.style={}
    }
\tikzset{
	thickness/.style={thick},
    operator/.style={draw,fill=white,minimum size=1.5em, inner sep=2pt,thickness,align=center},
    ggroup/.style={draw,minimum size=1.5em,thickness,align=center,inner sep=4pt},
    leftinternal/.style={anchor=mid west,font=\scriptsize,inner sep=4pt,align=center},
    rightinternal/.style={anchor=mid east,font=\scriptsize,inner sep=4pt,align=center},
    wave/.style={inner sep=-3pt,tape,fill=white,apply={draw=black} except on segments {5,6,1,2,9}},
    phase/.style={fill,shape=circle,minimum size=4pt},
    phase label/.style={label distance=2mm,anchor=mid,label position=45},
    ophase/.style={fill=white,draw=black,shape=circle,minimum size=4pt},
    internal/.style={thickness,black},
    line/.style={path picture={ 
\draw[internal](path picture bounding box.west) -- (path picture bounding box.east);
}},
	linecont/.style={circle,line},
    cross/.style={path picture={ 
\draw[internal](path picture bounding box.north) -- (path picture bounding box.south) (path picture bounding box.west) -- (path picture bounding box.east);
}},
    circlewc/.style={draw,circle,cross,minimum width=4pt,inner sep=3pt},
    crossx/.style={path picture={ 
\draw[internal,inner sep=0pt]
(path picture bounding box.south east) -- (path picture bounding box.north west) (path picture bounding box.south west) -- (path picture bounding box.north east) (path picture bounding box.west) -- (path picture bounding box.east);
}},
	crossx2/.style={circle,crossx,minimum size=1em},
    dd/.style={decoration={brace},decorate,thickness},
    dm/.style={decoration={brace,mirror},decorate,thickness},
    slice/.style={thickness,red,dash pattern=on 5pt off 3pt,align=center},
    meter/.style={draw,fill=white,minimum width=2em,minimum height=1.5em, rectangle, font=\vphantom{A}, thickness,
 path picture={\draw[black] ([shift={(.1,.24)}]path picture bounding box.south west) to[bend left=50] ([shift={(-.1,.24)}]path picture bounding box.south east);\draw[black,-{Latex[scale=0.6]}] ([shift={(0,.1)}]path picture bounding box.south) -- ([shift={(.3,-.1)}]path picture bounding box.north);}},
 	measuretab/.style={draw,signal,signal to=west,inner sep=4pt,fill=white},
 	meterD/.style={draw,rounded rectangle,rounded rectangle left arc=none,inner sep=4pt,fill=white},
 	measure/.style={draw,rounded rectangle,inner sep=4pt,fill=white},
 	my label/.style={yshift=0.1cm,above,align=center},
 	gg label/.style={label position=center,align=center},
 	group label/.style={label position=above,yshift=0.2cm,anchor=mid},
 	strike arrow/.style={
    decoration={markings, mark=at position 0.5 with {
        \draw [internal,-] 
            ++ (-\pgfkeysvalueof{/quantikz/Strike Width},-\pgfkeysvalueof{/quantikz/Strike Height} )
            -- ( \pgfkeysvalueof{/quantikz/Strike Width}, \pgfkeysvalueof{/quantikz/Strike Height});}	%can I use pgfkeys and do some maths here?
    },
    postaction={decorate},
}
}

\def\resetstyles{
\tikzcdset{thin,every cell/.append style={thin},arrows/.append style={thin}
    }
\tikzset{
	thickness/.style={thin},
	%operator/.append style={thin},
	%internal/.append style={thin},
	%dd/.append style={thin},
	%dm/.append style={thin},
	%slice/.append style={thin},
	meter/.append style={thin},
	phase/.append style={minimum size=3pt},
	ophase/.append style={minimum size=3pt},
	%circlewc/.append style={minimum size=3pt,inner sep=2pt}
}
}

\def\maketransparent{
\tikzset{
	operator/.append style={fill opacity=0},
	meter/.append style={fill opacity=0}
}
}
